Generalised norm resolvent convergence: comparison of different concepts

In this paper, we show that the two concepts of generalised norm resolvent convergence introduced by Weidmann and the first author of this paper are equivalent. We also focus on the convergence speed and provide conditions under which the convergence speed is the same for both concepts. We illustrate the abstract results by a large number of examples.

==> olafs_macros.tex <==
%------------------------------------------------------------------------
% olafs_macros.tex
%
% --- version 2015-11-27
%------------------------------------------------------------------------

\newcommand{\olafsMacrosIncluded}{} % flag to show if this file is included
%------------------------------------------------------------------------
% Packages and commands for layout
%------------------------------------------------------------------------

\usepackage{scrpage2}    % change headings, see Franzis book, p. 500)
\pagestyle{scrheadings}
%\typearea[7.5mm]{17}    % [BCOR Bindungskorrektur]{DIV=17 Einteilung der Seite}
\usepackage{scrtime}     % give time by \thistime

\usepackage{ifthen}       % used for ``draft'' mode

%------------------------------------------------------------------------
% Packages and commands for final version/draft version
%------------------------------------------------------------------------
\ifthenelse{\isundefined \finalVersion}
{ %% Draft mode: show remarks \look etc.
  % use headers with date and time
% one lines on top of page
  \rehead{\texttt{\jobname.tex}, \today, \thistime}
  \lohead{\texttt{\jobname.tex}, \today, \thistime}

% two lines on top of page
%  \rehead{\parbox[t]{0.3\textwidth}%   use
%    {\texttt{\jobname.tex}\\\today, \thistime}}
%  \lohead{\parbox[t]{0.3\textwidth}%
%    {\texttt{\jobname.tex}\\\today, \thistime}}


  \newcommand{\marker}[1]{\fbox{\rule{0pt}{0.1ex}\textbf{#1}}}
  \newcommand{\markerO}{\marker{Olaf}}
  \newcommand{\markerS}{\marker{Sebastian}}

  \newcounter{lookcounter}
  \setcounter{lookcounter}{0}
  \newcommand{\look}[2][$\diamond$]
             {
               \stepcounter{lookcounter}
               \marker{#1}
               \footnote[\arabic{lookcounter}]{\marker{$\diamond$} #2}
             }
  \newcommand{\lookO}[1]
             {
               \stepcounter{lookcounter}
               \markerO
               \footnote[\arabic{lookcounter}]{\markerO #1}
             }
  \newcommand{\lookS}[1]
             {
               \stepcounter{lookcounter}
               \markerS
               \footnote[\arabic{lookcounter}]{\markerS #1}
             }

  % show labels and show filename, date/time in headings (in draft mode)
  % load showkeys (I use a changed version with larger fonts)
  \ifthenelse{\isundefined \OlafsVersion}
  {\usepackage[notref,notcite]{showkeys}}              % on other computers
  {\usepackage{/home/post/Aktuell/LaTeX/my-showkeys}}  % on Olaf's computer
}
{ %% final mode: don't show remarks --- use standard headers
  \lohead{\textsf{\shorttitle}}
  \rehead{\textsf{\authors}}
  \automark[subsection]{section}
  \automark[subsection]{section}

  \newcommand{\look}[1]{}%
  \newcommand{\lookO}[1]{}%
  \newcommand{\lookS}[1]{}%
}

\newcommand{\comment}[1]{}   % put old stuff here (for debugging etc.)

%------------------------------------------------------------------------
% Package et al for graphics
%------------------------------------------------------------------------
\usepackage{graphicx}                % for graphics
%\newcommand{\color}[2][{}]{}         % figure-x.pstex_t file contains this

%------------------------------------------------------------------------
% Maths and other packages
%------------------------------------------------------------------------

\usepackage{amsmath, amssymb}%, theorem}
\usepackage{amsthm}

%\usepackage{diagrams}  % use diagrams
\usepackage{amscd}

%\usepackage{MnSymbol}    % for \llangle, \rrangle
  % has terrible side effects! no \colon, \setminus is bad etc!!!
  % don't need it anyway now ...

\usepackage{accents}     % for \accentset, \ring...
%\usepackage{yhmath}     % for \wideparen, ... (wide parenthesis over symbols)
   % not good: \widetilde looks quite ugly ...
\usepackage{mathtools}  % for \coloneqq etc.

\usepackage{bbm}         % blackboard (see: /usr/share/texmf/mytex/bbm.dvi)


\usepackage{mathrsfs}    % use ``real'' caligraphic letters for \mathcal
%\renewcommand \mathcal \mathscr

\usepackage{xspace}  % for adding space after macros automatically

%------------------------------------------------------------
% Equation numbering
%------------------------------------------------------------
\numberwithin{equation}{section}

%------------------------------------------------------------
% Enumerate numbering
%------------------------------------------------------------
% choose what you prefer ;-)
%\renewcommand{\theenumi}{\roman{enumi}} % (i), (ii) etc.
\renewcommand{\theenumi}{\alph{enumi}} % (a), (b) etc.
\renewcommand{\labelenumi}{(\theenumi)} % (i), (ii) etc.

%--------------------------------------------------------------------------
% Own enumerate environment (uses less space between items, no indent etc.)
%--------------------------------------------------------------------------
\newcounter{myenumi}
\newenvironment{myenumerate}[1]{
% begin
\begin{list}{\indent(\themyenumi) }
  {\renewcommand{\themyenumi}{#1{myenumi}}
    \usecounter{myenumi}
    \setlength{\topsep}{0em}
    \setlength{\itemsep}{0em}
    \setlength{\leftmargin}{0em}
    \setlength{\labelwidth}{0em}
    \setlength{\labelsep}{0em}}
  % \renewcommand{\makelabel}[1]{\textbf{\textsf{\large #1} }}
  }
  {
    % end
  \end{list}
  }

\newenvironment{myitemize}
{
  % begin
  \begin{list}{\indent $\bullet$}
  {
    \setlength{\topsep}{0.5em}
    \setlength{\itemsep}{0.0em}
    \setlength{\leftmargin}{2em}
    \setlength{\labelwidth}{3em}
    \setlength{\labelsep}{0.5em}
  }
}
{
  % end
  \end{list}
}


% own command for references of enumerate environments
\newcommand{\itemref}[1]{\eqref{#1}}


%------------------------------------------------------------
% theoremlike environments
%------------------------------------------------------------
% Change head font to sf:
\newcommand{\myfont}{\sffamily}
% Or leave it as it is:
%\renewcommand{\myfont}{}

\newcommand{\myparagraph}[1]{\noindent\textbf{\myfont{#1}}}

\newtheoremstyle{mythmstyle}% name
  {\topsep}% Space above1
  {\topsep}% Space below
  {\itshape}% Body font
  {}% Indent amount
  {\bfseries \myfont}% Theorem head font
  {.}%Punctuation after theorem head
  {.5em}%Space after theorem head
  {}% theorem head spec

\newtheoremstyle{mydefstyle}% name
  {\topsep}% Space above
  {\topsep}% Space below
  {\normalfont}% Body font
  {}% Indent amount
  {\bfseries \myfont}% Theorem head font
  {.}%Punctuation after theorem head
  {.5em}%Space after theorem head
  {}% theorem head spec

\swapnumbers                    % 1.1 Theorem instead of Theorem 1.1

\theoremstyle{mythmstyle}       % my style (new fonts) -- body italics

\newtheorem{theorem}{Theorem}[section]
\newtheorem{maintheorem}[theorem]{Main Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}

\newcounter{intro}
\renewcommand{\theintro}{\Alph{intro}}
\newtheorem{theo}[intro]{Theorem}
\newtheorem{df}[intro]{Definition}
\newtheorem{prop}[intro]{Proposition}
\newtheorem{coro}[intro]{Corollary}
%\newcounter{remintro}
%\renewcommand{\theremintro}{\Alph{remintro}}
%\newtheorem{remi}[remintro]{Remark 1.\!\!}

\newtheorem{conjecture}[theorem]{Conjecture}

\theoremstyle{mydefstyle}        % my style (new fonts) -- body roman
%\theoremstyle{definition}       % body roman
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{example}[theorem]{Example}
\newtheorem{examples}[theorem]{Examples}

%\theoremstyle{remark}   % uncomment if Remark and Notation appear
%                        % with italic name instead of bold
%   Actually, I don't like it ... so better leave it commented (op)
\newtheorem{remark}[theorem]{Remark}
\newtheorem{remarks}[theorem]{Remarks}
\newtheorem*{remark*}{Remark}
\newtheorem{notation}[theorem]{Notation}
%\newtheorem*{notation*}{Notation}

% Change font of "Proof":
% (see http://tex.stackexchange.com/questions/8089/changing-style-of-proof)
\expandafter\let\expandafter\oldproof\csname\string\proof\endcsname
\let\oldendproof\endproof
\renewenvironment{proof}[1][\bfseries\myfont\proofname]{%
  \oldproof[\bfseries \myfont #1]%
}{\oldendproof}

%------------------------------------------------------------
% Change of amsart.cls (section/subsection font and style etc.)
%------------------------------------------------------------

%\usepackage{etoolbox}
%\patchcmd{\section}{\bfseries\itshape}{\bfseries\itshape}{}{}
%\patchcmd{\subsection}{\bfseries\itshape}{\bfseries\itshape}{}{}
\makeatletter
\renewcommand\section{\@startsection{section}{1}%
  \z@{.7\linespacing\@plus\linespacing}{.5\linespacing}%
  {\Large\myfont\bfseries}}
  %{\normalfont\scshape\centering}}
\renewcommand\subsection{\@startsection{subsection}{2}%
  \z@{-.5\linespacing\@plus-.7\linespacing}{.5\linespacing}%
  {\large\myfont\bfseries}}
%  {\normalfont\bfseries}}
\renewcommand\subsubsection{\@startsection{subsubsection}{3}%
  \z@{.5\linespacing\@plus.7\linespacing}{-.5em}%
  {\myfont\bfseries}}
%  {\normalfont\itshape}}
\renewenvironment{abstract}{%
  \ifx\maketitle\relax
    \ClassWarning{\@classname}{Abstract should precede
      \protect\maketitle\space in AMS document classes; reported}%
  \fi
  \global\setbox\abstractbox=\vtop \bgroup
    \normalfont\Small
    \list{}{\labelwidth\z@
      \leftmargin3pc \rightmargin\leftmargin
      \listparindent\normalparindent \itemindent\z@
      \parsep\z@ \@plus\p@
      \let\fullwidthdisplay\relax
    }%
    \item[\hskip\labelsep%\scshape
      \myfont\bfseries
    \abstractname.]%
}{%
  \endlist\egroup
  \ifx\@setabstract\relax \@setabstracta \fi
}
\renewcommand\contentsnamefont{\myfont\bfseries}%{\scshape}
\renewcommand\@starttoc[2]{\begingroup
  \setTrue{#1}%
  \par\removelastskip\vskip\z@skip
  \@startsection{}\@M\z@{\linespacing\@plus\linespacing}%
    {.5\linespacing}{%\centering
      \contentsnamefont}{#2}%
  \ifx\contentsname#2%
  \else \addcontentsline{toc}{section}{#2}\fi
  \makeatletter
  \@input{\jobname.#1}%
  \if@filesw
    \@xp\newwrite\csname tf@#1\endcsname
    \immediate\@xp\openout\csname tf@#1\endcsname \jobname.#1\relax
  \fi
  \global\@nobreakfalse \endgroup
  \addvspace{32\p@\@plus14\p@}%
  \let\tableofcontents\relax
}
\renewcommand\@settitle{\begin{center}%
  \baselineskip14\p@\relax
    \LARGE
    \bfseries
    \myfont
%\uppercasenonmath
%    \@title
  \@title
  \end{center}%
}
\renewcommand\@setauthors{%
  \begingroup
  \def\thanks{\protect\thanks@warning}%
  \trivlist
  \centering\footnotesize \@topsep30\p@\relax
  \advance\@topsep by -\baselineskip
  \item\relax
  \author@andify\authors
  \def\\{\protect\linebreak}%
  %\MakeUppercase{\authors}%
  \large
  \myfont\bfseries\authors
  \ifx\@empty\contribs
  \else
    ,\penalty-3 \space \@setcontribs
    \@closetoccontribs
  \fi
  \endtrivlist
  \normalfont\myfont\@setaddresses
  \endgroup
}
\renewcommand\@setaddresses{\par
  \nobreak \begingroup
\footnotesize
  \def\author##1{\nobreak\addvspace\bigskipamount}%
  \def\\{\unskip, \ignorespaces}%
  \interlinepenalty\@M
  \def\address##1##2{\begingroup
    \par\addvspace\bigskipamount\indent
    \@ifnotempty{##1}{(\ignorespaces##1\unskip) }%
    {%\scshape
      \ignorespaces##2}\par\endgroup}%
  \def\curraddr##1##2{\begingroup
    \@ifnotempty{##2}{\nobreak\indent\curraddrname
      \@ifnotempty{##1}{, \ignorespaces##1\unskip}\/:\space
      ##2\par}\endgroup}%
  \def\email##1##2{\begingroup
    \@ifnotempty{##2}{\nobreak\indent\emailaddrname
      \@ifnotempty{##1}{, \ignorespaces##1\unskip}\/:\space
      \ttfamily##2\par}\endgroup}%
  \def\urladdr##1##2{\begingroup
    \def~{\char`\~}%
    \@ifnotempty{##2}{\nobreak\indent\urladdrname
      \@ifnotempty{##1}{, \ignorespaces##1\unskip}\/:\space
      \ttfamily##2\par}\endgroup}%
  \addresses
  \endgroup
}
\renewcommand\enddoc@text{\ifx\@empty\@translators \else\@settranslators\fi
  %\ifx\@empty\addresses \else\@setaddresses\fi
}
\renewcommand\@secnumfont{\myfont\bfseries} %{\mdseries}

\renewcommand\maketitle{\par
  \@topnum\z@ % this prevents figures from falling at the top of page 1
  \@setcopyright
  \thispagestyle{firstpage}% this sets first page specifications
%  \uppercasenonmath\shorttitle
  \ifx\@empty\shortauthors \let\shortauthors\shorttitle
  \else \andify\shortauthors
  \fi
  \@maketitle@hook
  \begingroup
  \@maketitle
  \toks@\@xp{\shortauthors}\@temptokena\@xp{\shorttitle}%
  \toks4{\def\\{ \ignorespaces}}% defend against questionable usage
  \edef\@tempa{%
    \@nx\markboth{\the\toks4
      \@nx\MakeUppercase{\the\toks@}}{\the\@temptokena}}%
  \@tempa
  \endgroup
  \c@footnote\z@
  \@cleartopmattertags
}
\makeatother
%------------------------------------------------------------
% End of changes of amsart.cls
%------------------------------------------------------------

%------------------------------------------------------------
% References unified
%------------------------------------------------------------
% Why this?
% If you for some reason change a Prop. into a Lemma, then "we
% refer to Lemma~\ref{prp:blabla}" wont see this, but "we refer to
% \Lem{blabla}" (assuming that Lemmas have label "lem:blabla" and
% Prop. have labels "prp:blabla" ;-) (op)
%
% Sections etc.
\newcommand{\Sec}[1]{Section~\ref{sec:#1}}
\newcommand{\Secs}[2]{Sections~\ref{sec:#1} and~\ref{sec:#2}}
\newcommand{\App}[1]{Appendix~\ref{app:#1}}
\newcommand{\Apps}[2]{Appendices~\ref{app:#1} and~\ref{app:#2}}
\newcommand{\Subsec}[1]{Subsection~\ref{ssec:#1}}
\newcommand{\Subsecs}[2]{Subsections~\ref{ssec:#1} and~\ref{ssec:#2}}
\newcommand{\SubsecS}[2]{Subsections~\ref{ssec:#1}--\ref{ssec:#2}}

% Equations:
\newcommand{\Eq}[1]{Eq.~\eqref{eq:#1}}
\newcommand{\Eqs}[2]{Eqs.~\eqref{eq:#1} and~\eqref{eq:#2}}
\newcommand{\EqS}[2]{Eqs.~\eqref{eq:#1}--\eqref{eq:#2}}

% Figures
\newcommand{\Fig}[1]{Figure~\ref{fig:#1}}
\newcommand{\Figenum}[2]{Figure~\ref{fig:#1}~(\ref{#2})}
\newcommand{\Figs}[2]{Figures~\ref{fig:#1} and~\ref{fig:#2}}

% Footnotes
\newcommand{\Footnote}[1]{Footnote~\ref{fn:#1}}
\newcommand{\Footnotes}[2]{Footnotes~\ref{fn:#1} and~\ref{fn:#2}}
\newcommand{\FootnoteS}[2]{Footnotes~\ref{fn:#1}--\ref{fn:#2}}

% Theoremlike environments:
\newcommand{\Thm}[1]{Theorem~\ref{thm:#1}}
\newcommand{\Thms}[2]{Theorems~\ref{thm:#1} and~\ref{thm:#2}}
\newcommand{\ThmS}[2]{Theorems~\ref{thm:#1}--\ref{thm:#2}}
\newcommand{\Thmenum}[2]{Theorem~\ref{thm:#1}~(\ref{#2})}
\newcommand{\Thmenums}[3]{Theorem~\ref{thm:#1}~(\ref{#2}) and~(\ref{#3})}
\newcommand{\ThmenumS}[3]{Theorem~\ref{thm:#1}~(\ref{#2})--(\ref{#3})}
%\newcommand{\AssThmenum}[2]{Assumption~(\ref{#2}) of Theorem~\ref{thm:#1}~}

\newcommand{\Ex}[1]{Example~\ref{ex:#1}}
\newcommand{\Exs}[2]{Examples~\ref{ex:#1} and~\ref{ex:#2}}
\newcommand{\ExS}[2]{Examples~\ref{ex:#1}--\ref{ex:#2}}
\newcommand{\Exenum}[2]{Example~\ref{ex:#1}~(\ref{#2})}
\newcommand{\Exenums}[3]{Example~\ref{ex:#1}~(\ref{#2}) and~(\ref{#3})}
\newcommand{\ExenumS}[3]{Example~\ref{ex:#1}~(\ref{#2})--(\ref{#3})}

\newcommand{\Lem}[1]{Lemma~\ref{lem:#1}}
\newcommand{\Lems}[2]{Lemmata~\ref{lem:#1} and~\ref{lem:#2}}
\newcommand{\LemS}[2]{Lemmata~\ref{lem:#1}--\ref{lem:#2}}
\newcommand{\Lemenum}[2]{Lemma~\ref{lem:#1}~(\ref{#2})}
\newcommand{\Lemenums}[3]{Lemma~\ref{lem:#1}~(\ref{#2}) and~(\ref{#3})}
\newcommand{\LemenumS}[3]{Lemma~\ref{lem:#1}~(\ref{#2})--(\ref{#3})}

\newcommand{\Cor}[1]{Corollary~\ref{cor:#1}}
\newcommand{\Cors}[2]{Corollaries~\ref{cor:#1} and~\ref{cor:#2}}
\newcommand{\CorS}[2]{Corollaries~\ref{cor:#1}--\ref{cor:#2}}
\newcommand{\Corenum}[2]{Corollary~\ref{cor:#1}~(\ref{#2})}
\newcommand{\Corenums}[3]{Corollary~\ref{cor:#1}~(\ref{#2}) and~(\ref{#3})}
\newcommand{\CorenumS}[3]{Corollary~\ref{cor:#1}~(\ref{#2})--(\ref{#3})}

\newcommand{\Prp}[1]{Proposition~\ref{prp:#1}}
\newcommand{\Prps}[2]{Propositions~\ref{prp:#1} and~\ref{prp:#2}}
\newcommand{\PrpS}[2]{Propositions~\ref{prp:#1}--\ref{prp:#2}}
\newcommand{\Prpenum}[2]{Proposition~\ref{prp:#1}~(\ref{#2})}
\newcommand{\Prpenums}[3]{Proposition~\ref{prp:#1}~(\ref{#2}) and~(\ref{#3})}
\newcommand{\PrpenumS}[3]{Proposition~\ref{prp:#1}~(\ref{#2})--(\ref{#3})}

\newcommand{\Rem}[1]{Remark~\ref{rem:#1}}
\newcommand{\Rems}[2]{Remarks~\ref{rem:#1} and~\ref{rem:#2}}
\newcommand{\RemS}[2]{Remarks~\ref{rem:#1}--\ref{rem:#2}}
\newcommand{\Remenum}[2]{Remark~\ref{rem:#1}~(\ref{#2})}
\newcommand{\Remenums}[3]{Remark~\ref{rem:#1}~(\ref{#2}) and~(\ref{#3})}
\newcommand{\RemenumS}[3]{Remark~\ref{rem:#1}~(\ref{#2})--(\ref{#3})}

\newcommand{\Def}[1]{Definition~\ref{def:#1}}
\newcommand{\Defs}[2]{Definitions~\ref{def:#1} and~\ref{def:#2}}
\newcommand{\Defss}[3]{Definitions~\ref{def:#1}, ~\ref{def:#2} and~\ref{def:#3}}
\newcommand{\DefS}[2]{Definitions~\ref{def:#1}--\ref{def:#2}}
\newcommand{\Defenum}[2]{Definition~\ref{def:#1}~(\ref{#2})}
\newcommand{\Defenums}[3]{Definition~\ref{def:#1}~(\ref{#2}) and~(\ref{#3})}
\newcommand{\DefenumS}[3]{Definition~\ref{def:#1}~(\ref{#2})--(\ref{#3})}

\newcommand{\Ass}[1]{Assumption~\ref{ass:#1}}
\newcommand{\Asss}[2]{Assumptions~\ref{ass:#1} and~\ref{ass:#2}}
\newcommand{\AssS}[2]{Assumptions~\ref{ass:#1}--\ref{ass:#2}}
\newcommand{\Assenum}[2]{Assumption~\ref{ass:#1}~(\ref{#2})}
\newcommand{\Assenums}[3]{Assumption~\ref{ass:#1}~(\ref{#2}) and~(\ref{#3})}
\newcommand{\AssenumS}[3]{Assumption~\ref{ass:#1}~(\ref{#2})--(\ref{#3})}

\newcommand{\Not}[1]{Notation~\ref{not:#1}}
\newcommand{\Nots}[2]{Notations~\ref{not:#1} and~\ref{not:#2}}
\newcommand{\NotS}[2]{Notations~\ref{not:#1}--\ref{not:#2}}
\newcommand{\Notenum}[2]{Notation~\ref{not:#1}~(\ref{#2})}
\newcommand{\Notenums}[3]{Notation~\ref{not:#1}~(\ref{#2}) and~(\ref{#3})}
\newcommand{\NotenumS}[3]{Notation~\ref{not:#1}~(\ref{#2})--(\ref{#3})}


%------------------------------------------------------------
%
% Mathematical definitions
%
%------------------------------------------------------------

%------------------------------------------------------------
% norms and squared norms
%------------------------------------------------------------
\newcommand{\abs}[2][{}]{\lvert{#2}\rvert_{{#1}}}    % abs value
\newcommand{\abssqr}[2][{}]{\lvert{#2}\rvert^2_{#1}} % abs squared
\newcommand{\bigabs}[2][{}]{\bigl\lvert{#2}\bigr\rvert_{#1}}     % abs
\newcommand{\bigabssqr}[2][{}]{\bigl\lvert{#2}\bigr\rvert^2_{#1}}% abs squared
\newcommand{\Bigabs}[2][{}]{\Bigl\lvert{#2}\Bigr\rvert_{#1}}     % abs
\newcommand{\Bigabssqr}[2][{}]{\Bigl\lvert{#2}\Bigr\rvert^2_{#1}}% abs squared
\newcommand{\BIGabs}[2][{}]{\left\lvert{#2}\right\rvert_{#1}}     % abs
\newcommand{\BIGabssqr}[2][{}]{\left\lvert{#2}\right\rvert^2_{#1}}% abs squared

% define this only at one instance of the file!
\newcommand{\normsymb}{\|}
\newcommand{\bignormsymb}[1]{#1\|}
%\newcommand{\bignormsymb}[1]{#1|\!#1|}

\newcommand{\norm}[2][{}]{\normsymb{#2}\normsymb_{{#1}}}    % norm
\newcommand{\normsqr}[2][{}]{\normsymb{#2}\normsymb^2_{#1}} % norm squared
\newcommand{\bignorm}[2][{}]{\bignormsymb{\bigl}{#2}\bignormsymb{\bigr}_{#1}}
\newcommand{\bignormsqr}[2][{}]{\bignormsymb{\bigl}{#2}%
                                \bignormsymb{\bigr}^2_{#1}}% norm squared
\newcommand{\Bignorm}[2][{}]{\bignormsymb{\Bigl}{#2}\bignormsymb{\Bigr}_{#1}}
\newcommand{\Bignormsqr}[2][{}]{\bignormsymb{\Bigl}{#2}%
                                \bignormsymb{\Bigr}^2_{#1}}% norm squared
\newcommand{\BIGnorm}[2][{}]{\bignormsymb{\left}{#2}\Bignormsymb{\right}_{#1}}
\newcommand{\BIGnormsqr}[2][{}]{\bignormsymb{\left}{#2}%
                                \bignormsymb{\right}^2_{#1}}% norm squared

%------------------------------------------------------------
% inner products
%------------------------------------------------------------
\newcommand{\iprod}[3][{}]{\langle{#2},{#3}\rangle_{#1}}  % inner product
\newcommand{\bigiprod}[3][{}]{\bigl\langle{#2},{#3}\bigr\rangle_{#1}}
\newcommand{\Bigiprod}[3][{}]{\Bigl\langle{#2},{#3}\Bigr\rangle_{#1}}


%------------------------------------------------------------
% topological/set symbols
%------------------------------------------------------------
\newcommand{\set}[2]{\{ \, #1 \, | \, #2 \, \} }      % set { #1 | #2 }
\newcommand{\bigset}[2]{\bigl\{ \, #1 \, \bigl|\bigr. \, #2 \, \bigr\} }
\newcommand{\Bigset}[2]{\Bigl\{ \, #1 \, \Bigl|\Bigr. \, #2 \, \Bigr\} }

\DeclareMathOperator*{\bigdcup}{\mathaccent\cdot{\bigcup}}
\DeclareMathOperator*{\dcup}   {\mathaccent\cdot\cup}

\newcommand{\map}[3]{ #1 \colon #2 \longrightarrow #3}    % maps
\newcommand{\embmap}[3]{ #1 \colon #2 \hookrightarrow #3} % embedding map

\newcommand{\bd}  {\partial}          % symbol for boundary of a set
\newcommand{\clo}[2][]{\overline{{#2}}^{#1}} %  symbol for closure
\newcommand{\intr}[1]{\ring{{#1}}}    %  symbol for interior

\newcommand{\restr}[1]{{\restriction}_{#1}} % symbol for map restriction

%------------------------------------------------------------
% integral with -
%------------------------------------------------------------
%
% code from file ``latex-symbols.pdf''
%------------------------------------------------------------
\def\Xint#1{\mathchoice
   {\XXint\displaystyle\textstyle{#1}}%
   {\XXint\textstyle\scriptstyle{#1}}%
   {\XXint\scriptstyle\scriptscriptstyle{#1}}%
   {\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
   \!\int}
\def\XXint#1#2#3{{\setbox0=\hbox{$#1{#2#3}{\int}$}
     \vcenter{\hbox{$#2#3$}}\kern-.5\wd0}}
\def\XXsum#1#2#3{{\setbox0=\hbox{$#1{#2#3}{\int}$}
     \vcenter{\hbox{$#2#3$}}\kern-.60\wd0}}
\def\Xsum#1{\mathchoice
   {\XXsum\displaystyle\textstyle{#1}}%
   {\XXsum\textstyle\scriptstyle{#1}}%
   {\XXsum\scriptstyle\scriptscriptstyle{#1}}%
   {\XXsum\scriptscriptstyle\scriptscriptstyle{#1}}%
   \!\sum}
\newcommand{\ddashint}{\Xint=}
\newcommand{\dashint}{\Xint-}   % \int with -
\newcommand{\dashsum}{\Xsum-}   % \sum with -
\newcommand{\avint}{{\textstyle\dashint}}   % average sum
\newcommand{\avsum}[1][{}]{{}^{#1}\text-\hspace*{-1ex}\Sigma}   % average sum

%------------------------------------------------------------
% Math names
%------------------------------------------------------------

\newcommand{\card}[1]{\lvert#1\rvert}   % from AMS proceedings file
                                        % Here for cardinality of a set
\DeclareMathOperator{\const}  {const}
%\DeclareMathOperator{\dd}    {d\!}
\newcommand{\dd}    {\, \mathrm d}    % not optimal: no \, if at beginning
%\DeclareMathOperator{\dist}   {dist}
\DeclareMathOperator{\diam}   {diam}
\DeclareMathOperator{\dom}    {dom}
\DeclareMathOperator{\ran}    {ran}
\DeclareMathOperator{\id}     {id}   % identity map
\DeclareMathOperator{\ind}    {ind}  % index
\DeclareMathOperator{\injrad} {inj\,rad}
%\DeclareMathOperator{\intr}   {int}  % topological interiour
\DeclareMathOperator{\Ric}    {Ric}
\DeclareMathOperator{\Scal}   {Scal}
\DeclareMathOperator{\sgn}    {sgn}
\DeclareMathOperator{\supp}   {supp}
\DeclareMathOperator{\vol}    {vol}
\DeclareMathOperator{\dvol}    {d\, vol}
\DeclareMathOperator{\tr}     {tr}  % trace

\DeclareMathOperator{\Hom}    {Hom}


\newcommand{\de} {\mathord{\mathrm d}} % exterior derivative

\newcommand{\specsymb} {\sigma} % symbol for spectrum

\newcommand{\spec}[2][{}]   {\specsymb_{\mathrm{#1}}(#2)}
\newcommand{\bigspec}[2][{}]   {\specsymb_{\mathrm{#1}}\bigl(#2\bigr)}
\newcommand{\Bigspec}[2][{}]   {\specsymb_{\mathrm{#1}}\Bigl(#2\Bigr)}
\newcommand{\essspec}[1]{\spec[ess] {#1}}
\newcommand{\disspec}[1]{\spec[disc]{#1}}

%------------------------------------------------------------
% replace some ugly standard LaTeX symbols and letters
%------------------------------------------------------------

\newcommand{\eps}{\varepsilon} % shortcut
\renewcommand{\phi}{\varphi}   % shortcut
\renewcommand{\rho}{\varrho}   % shortcut
%\renewcommand{\theta}{\vartheta}% shortcut

% The next is how to redefine \Re, but using DeclareMathOperator!
\DeclareMathOperator{\myRe} {Re}
\renewcommand{\Re}     {\myRe}
\DeclareMathOperator{\myIm}     {Im}
\renewcommand{\Im}     {\myIm}

\newcommand{\conj}[1]{\overline {#1}}
                    % symbol for complex conjugation


%------------------------------------------------------------
% general math shortcuts
%------------------------------------------------------------
\newcommand{\R}{\mathbb{R}} % symbol for real numbers
\newcommand{\C}{\mathbb{C}} % symbol for complex numbers
\newcommand{\N}{\mathbb{N}} % symbol for natural numbers
\newcommand{\Z}{\mathbb{Z}} % symbol for integers
\newcommand{\Sphere}{\mathbb{S}} % symbol for sphere
\newcommand{\Torus}{\mathbb{T}} % symbol for torus

%\newcommand{\1}{\mathbf 1}                  % if bbm does'nt work
\newcommand{\1}{\mathbbm 1}                    % blackboard 1

\newcommand{\e}{\mathrm e}  %Euler number
\newcommand{\im}{\mathrm i} % complex unit

\newcommand{\normder}{\partial_\mathrm{n}}  % symbol for normal derivative

%------------------------------------------------------------
% general font/attributes
%------------------------------------------------------------
\newcommand{\wt}{\widetilde}           % shortcut
\newcommand {\qf}[1]{\mathfrak{#1}}    % font for quadratic forms

\newcommand{\leCS}{\stackrel{\mathrm{CS}}\le}
\newcommand{\leCY}{\stackrel{\mathrm{CY}}\le}
\newcommand{\geCS}{\stackrel{\mathrm{CS}}\ge}
\newcommand{\geCY}{\stackrel{\mathrm{CY}}\ge}

%------------------------------------------------------------
% Banach spaces
%------------------------------------------------------------
\newcommand{\HS}{\mathscr H}           % symbol for Hilbert space
%\newcommand{\HS}{\mathsf H}           % symbol for Hilbert space
\newcommand{\HSaux}{\mathscr G}        % symbol for auxiliary Hilbert space
%\newcommand{\HSaux}{\mathsf G}        % symbol for auxiliary Hilbert space
\newcommand{\HSn}{\ring \HS}

\newcommand{\Sobsymb} {\mathsf H} % symbol for Sobolev space
\newcommand{\Sobnsymb} {\ring{\mathsf H}} % symbol for Sobolev space
\newcommand{\SobWsymb}{\mathsf W} % symbol for Sobolev-W space
\newcommand{\SobnWsymb}{\ring{\mathsf W}} % symbol for Sobolev-W space

\newcommand{\Contsymb} {\mathsf C}     % symbol for cont. space
\newcommand{\Lsymb}    {\mathsf L}     % symbol for int L-spaces
\newcommand{\lsymb}    {\ell}          % symbol for int l-spaces

\newcommand{\TRspace}{\BdOpsymb_1}% symbol for trace class
\newcommand{\HSspace}{\BdOpsymb_2}% symbol for Hilbert-Schmidt class

%------------------------------------------------------------
% Symbols for functional spaces without space argument (add ..space to label)
%------------------------------------------------------------

\newcommand{\Sobspace}[1][1]{\Sobsymb^{#1}}
  % symbol for Sobolev space
  % usage: \Sobspace [k] -> H^k
\newcommand{\Sobnspace}[1][1]{\Sobnsymb^{#1}}

\newcommand{\SobWspace}[2][p]{\SobWsymb_{#1}^{#2}}
\newcommand{\SobnWspace}[2][p]{\SobnWsymb_{#1}^{#2}}
  % symbol for Sobolev-W space
  % usage: e.g. \SobWspace[p,\loc] k gives W_{p,\loc}^k
\newcommand{\Contspace}[1][{}]{\Contsymb^{#1}}     % symbol for cont. space
\newcommand{\Contlocspace}[1][{}]{\Contsymb^{#1}_\loc} % symbol for cont. space
\newcommand{\Lpspace}[1][p]    {\Lsymb_{#1}}     % symbol for int L-spaces
\newcommand{\lpspace}[1][p]    {\lsymb_{#1}}     % symbol for int L-spaces
\newcommand{\Lsqrspace}    {\Lpspace[2]}     % symbol for int L-spaces
\newcommand{\lsqrspace}    {\lpspace[2]}          % symbol for int l-spaces
\newcommand{\Linftyspace}    {\Lpspace[\infty]}     % symbol for int L-spaces
\newcommand{\linftyspace}    {\lpspace[\infty]}          % symbol for int l-spaces


\newcommand{\BdOpsymb} {\mathcal B}       % symbol for bounded linear operators
\newcommand{\BdOp}[2][{}]{\BdOpsymb_{#1}({#2})}
                                  %  symbol for bdd linear operators
\newcommand{\Unitary}[1]{\mathcal U({#1})}
                                  %  symbol for unitary operators



%------------------------------------------------------------
% spaces of continuous functions
%------------------------------------------------------------
\newcommand{\Ci} [2][{}]{\Contspace [\infty]_{#1} ({#2})}
                                       % C^\infty(#1)-spaces
\newcommand{\Cci}[1]{\Ci[\mathrm c]{#1}}%{\Contsymb^\infty_{\mathrm c} ({#1})}
                                       % C_c^\infty(#1)-sp
\newcommand{\Cont}[2][{}]{\Contspace[#1]({#2})}
                                       % space of cont (C^k) functions
\newcommand{\Contb}[2][{}]{\Contspace[#1]_{\mathrm b}({#2})}
                                       % space of C^k-bounded functions
\newcommand{\Contc}[2][{}]{\Contspace[#1]_{\mathrm c}({#2})}
                                       % space of C^k fct. wit compact supp
\newcommand{\Contloc}[2][{}]{\Contlocspace[#1]({#2})}
                                       % space of loc cont (C^k) functions

\newcommand{\Schwartz}[1]{\mathcal S(#1)}
%------------------------------------------------------------
% L_p-spaces
%------------------------------------------------------------
\newcommand{\Lp}[2][p]{\Lpspace [#1]({#2})} % L_#1(#2)-spaces
\newcommand{\Lploc}[2][p]{\Lpspace [#1,\mathrm{loc}]({#2})}
                                       % same, but loc
\newcommand{\lp}[2][p]{\lpspace [#1]({#2})} % l_#1(#2)-spaces

\newcommand{\Lsqr}[2][{}]{\Lsqrspace^{#1}({#2})} % L_2^{#1}(#2)-spaces
                                       % (with optional subscript
\newcommand{\Lsqrx}[2][{}]{\Lpspace [2,\mathrm{#1}]({#2})} %

\newcommand{\Lsqrloc}[2][{}]{\Lpspace [2,\mathrm{loc}]^{#1}({#2})}
                                       % L_{2,loc}(#1)-spaces
\newcommand{\lsqr}[2][{}]{\lsqrspace^{#1}({#2})}   % l_2(#1)-spaces

\newcommand{\Linfty}[2][{}]{\Lpspace [\infty] ^{#1}({#2})} % L_2(#1)-spaces
                                       % (with optional subscript
\newcommand{\Linftyloc}[2][{}]{\Lpspace [\infty,\mathrm{loc}]^{#1} ({#2})}
                                       % L_{\infty,loc}(#1)-spaces
\newcommand{\linfty}[1]{\lpspace [\infty] ({#1})}    % l_\infty(#1)-spaces

%------------------------------------------------------------
% Sobolev spaces
%------------------------------------------------------------
\newcommand{\Sob}[2][1]{\Sobspace [#1]({#2})}         % Sobolev space
\newcommand{\Sobn}[2][1]{\Sobnspace [#1]({#2})}  % Sob space ^0

\newcommand{\Sobx}[3][1]{\Sobspace [#1]_{{#2}}({#3})} % Sobolev space
\newcommand{\SobW}[3][p]{\SobWspace[#1]{#2}(#3)} % Sobolev W-space

\newcommand{\SobnW}[3][p]{\SobnWspace[#1]{#2}(#3)} % Sobolev W-space
%\newcommand{\Sobloc}[2][1]{\Sobx[#1]{\mathrm{loc}}{#2}}
                                                     % local Sobolev space
%\newcommand{\SobWloc}[2][1]{\SobWx[#1]{\mathrm{loc}}{#2}}


%------------------------------------------------------------
% Symbols for Laplacians
%------------------------------------------------------------
\newcommand{\Neu}{{\mathrm N}}              % symbol for Neumann bd cond
\newcommand{\Dir}{{\mathrm D}}              % symbol for Dirichlet bd cond
\newcommand{\NeuDir}{{\Neu \Dir}}             % symbol for mixed bd cond
\newcommand{\DirNeu}{{\Dir \Neu}}             % symbol for mixed bd cond
\newcommand{\laplacian}[2][{}]{\Delta_{{#2}}^{{#1}}}
                                             % symbol for Laplacian on mfd
\newcommand{\laplacianD}[1]{\laplacian[\Dir]{#1}} % symb f Dir-Laplacian
\newcommand{\laplacianN}[1]{\laplacian[\Neu]{#1}} % symb f Neu-Laplacian
\newcommand{\laplacianND}[1]{\laplacian[\NeuDir]{#1}} % symb f ND-Laplacian


%------------------------------------------------------------
% Symbol for error "O"
%------------------------------------------------------------
\newcommand{\err}{\mathrm o}  % not used ... better font!
\newcommand{\Err}{\mathrm O}


%------------------------------------------------------------
% some labels for math text (in \mathrm!!!)
%------------------------------------------------------------
\newcommand {\loc}{\mathrm{loc}}

%------------------------------------------------------------
% Other useful definitions
%------------------------------------------------------------
\newcommand{\quadtext}[1]{\quad\text{#1}\quad}
\newcommand{\qquadtext}[1]{\qquad\text{#1}\qquad}

%------------------------------------------------------------
%
% End of mathematical definitions
%
%------------------------------------------------------------

